Enhancing Incomplete Multi-modal Brain Tumor Segmentation with Intra-modal Asymmetry and Inter-modal Dependency

Deep learning-based brain tumor segmentation (BTS) models for multi-modal MRI images have seen significant advancements in recent years. However, a common problem in practice is the unavailability of some modalities due to varying scanning protocols and patient conditions, making segmentation from incomplete MRI modalities a challenging issue. Previous methods have attempted to address this by fusing accessible multi-modal features, leveraging attention mechanisms, and synthesizing missing modalities using generative models. However, these methods ignore the intrinsic problems of medical image segmentation, such as the limited availability of training samples, particularly for cases with tumors. Furthermore, these methods require training and deploying a specific model for each subset of missing modalities. To address these issues, we propose a novel approach that enhances the BTS model from two perspectives. Firstly, we introduce a pre-training stage that generates a diverse pre-training dataset covering a wide range of different combinations of tumor shapes and brain anatomy. Secondly, we propose a post-training stage that enables the model to reconstruct missing modalities in the prediction results when only partial modalities are available. To achieve the pre-training stage, we conceptually decouple the MRI image into two parts: `anatomy' and `tumor'. We pre-train the BTS model using synthesized data generated from the anatomy and tumor parts across different training samples. ... Extensive experiments demonstrate that our proposed method significantly improves the performance over the baseline and achieves new state-of-the-art results on three brain tumor segmentation datasets: BRATS2020, BRATS2018, and BRATS2015.

==> Figures/Additional_peer_comparison.tex <==
\begin{figure*}[ht]
  \centering
    \includegraphics[width=0.99\linewidth]{Pics/Additional_Peer_Comparison.pdf}
    \caption{Additional visualization of segmentation results between our method and state-of-the-art methods. From left to right, we demonstrate the MRI images for Flair modality, T1ce modality, T1 modality and T2 modality. Following the ground truth, the prediction of U-HVED\cite{dorent2019hetero}, RobustSeg\cite{chen2019robust}, RFNet\cite{ding2021rfnet} and our prediction. 
    }
    \label{Figure: Additional_peer_comparison}
\end{figure*}

==> Figures/Additional_post-training.tex <==
\begin{figure*}[ht]
  \centering
    \includegraphics[width=0.7\linewidth]{Pics/Additional_Post-training.pdf}
    \caption{Additional visualization of the prediction of different iterations for the KD-based post-training, while only T1 modality is input into the networks for prediction.}
    \label{Figure: Additional_post-training}
\end{figure*}

==> Figures/First_pipeline.tex <==
\begin{figure*}[t]
  \centering
    \includegraphics[width=\linewidth]{Pics/bts_teaser.pdf}
    \caption{The overall pipeline of our method. }
    \label{Fig: pipeline}
\end{figure*}

==> Figures/Probability_Features.tex <==
\begin{figure}[ht]
  \centering
    \includegraphics[width=\linewidth]{Pics/fig-probality-features.PNG}
    \caption{The Student network.  $prm\_pred1$, $prm\_pred2$, $prm\_pred3$, $prm\_pred4$ are features that correspond to the regional probability distribution map obtained by the teacher using the existing features. }
    \label{Figure-Probability-Features}
\end{figure}

==> Figures/predict_on_synthetic_samples.tex <==
\begin{figure*}[ht]
  \centering
    \includegraphics[width=1\linewidth]{Pics/predict_on_synthetic_samples.pdf}
    \caption{Different approaches' performance on synthetic samples. We marked out the tumor part added by asymmetric error maps with a yellow box on ground truth.}
    \label{Figure: predict_on_synthetic_samples}
\end{figure*}

==> Tables/abalation_augmentation_whole.tex <==
% \begin{table}[]
% \centering
% \small
% \resizebox{1.0\linewidth}{!}{
% \begin{tabular}{ccccccccccccc}
% \multicolumn{4}{c}{\textbf{Modalities}} & \multicolumn{9}{c}{\textbf{Whole}} \\
% \textbf{F} & \textbf{T1} & \textbf{Tc} & \textbf{T2} & \textbf{BL} & \textbf{+MU} & \textbf{+SA} & \textbf{RS} & \textbf{+MU} & \textbf{+SA} & \textbf{U-H} & \textbf{+MU} & \textbf{+SA} \\
% \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\bullet$} & 85.79 & 86.84 & 87.14 & 83.46 & 84.58 & 85.33 & 77.34 &  & 83.01 \\
% \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\circ$} & 76.51 & 78.57 & 80.46 & 70.49 & 73.64 & 74.31 & 62.88 &  & 69.40 \\
% \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\circ$} & 75.47 & 78.66 & 79.94 & 65.78 & 70.13 & 71.46 & 59.18 &  & 68.93 \\
% \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\circ$} & 86.96 & 87.59 & 87.83 & 83.69 & 84.65 & 84.91 & 79.22 &  & 82.99 \\
% \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\bullet$} & 87.96 & 88.19 & 88.80 & 86.57 & 87.37 & 87.57 & 80.31 &  & 83.95 \\
% \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\circ$} & 79.97 & 81.16 & 82.86 & 74.65 & 77.99 & 78.69 & 66.69 &  & 73.68 \\
% \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\circ$} & 89.80 & 90.05 & 90.09 & 87.09 & 88.21 & 88.13 & 81.74 &  & 85.42 \\
% \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\bullet$} & 87.90 & 88.13 & 88.48 & 85.63 & 86.93 & 87.29 & 79.82 &  & 84.23 \\
% \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\bullet$} & 89.88 & 89.94 & 90.38 & 88.37 & 88.27 & 89.02 & 82.78 &  & 86.68 \\
% \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\circ$} & 89.41 & 89.90 & 90.54 & 87.79 & 88.45 & 88.72 & 82.42 &  & 85.43 \\
% \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\circ$} & 90.20 & 90.66 & 91.06 & 88.28 & 89.23 & 89.46 & 83.31 &  & 85.98 \\
% \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\bullet$} & 90.48 & 90.55 & 90.70 & 88.83 & 89.44 & 89.68 & 83.71 &  & 87.25 \\
% \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\bullet$} & 90.56 & 90.82 & 91.08 & 89.49 & 89.81 & 90.10 & 84.14 &  & 87.13 \\
% \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\bullet$} & 88.59 & 88.81 & 89.24 & 86.46 & 87.83 & 87.93 & 81.09 &  & 84.15 \\
% \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\bullet$} & 90.97 & 90.99 & 91.27 & 89.54 & 90.34 & 90.41 & 84.56 &  & 87.19 \\
% \multicolumn{4}{c}{\textbf{Average}} & 86.70 & 87.39 & 87.99 & 83.75 & 85.12 & 85.53 & 77.95 &  & 82.36
% \end{tabular}
% }
% \end{table}

==> Tables/ablation_KD_detail_RFNet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\large
\renewcommand\arraystretch{1} 
\caption{The ablation study to evaluate the impact of increasing the training iterations of the knowledge distillation (KD)-based post-training method. We denote the models post-trained with $N$ epochs using the KD approach as KD-$N$. We compared the performance of our proposed method to the RFNet\cite{ding2021rfnet} baseline. Results are reported using the Dice Score (\%) metric with BRATS2020. The available and missing modalities are denoted by \textbf{$\bullet$} and \textbf{$\circ$}, respectively.}
\begin{adjustbox}{width=2\columnwidth,center}
\begin{tabular}{cccc|cccc|cccc|cccc}
\toprule
\multicolumn{4}{c|}{}                                                                                                                                  & \multicolumn{12}{c}{\textbf{Dice score(\%)}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{5-16} 
\multicolumn{4}{c|}{\multirow{-2}{*}{\textbf{Modality}}}                                                                                               & \multicolumn{4}{c|}{\textbf{Whole}}                                                                                                                                                                        & \multicolumn{4}{c|}{\textbf{Core}}                                                                                                                                                                         & \multicolumn{4}{c}{\textbf{Enhancing}}                                                                                                                                                                     \\
\midrule
  
\textbf{Flair} & \textbf{T1} & \textbf{T1ce} & \textbf{T2} & \textbf{RF+AEM} & \textbf{KD-300} & \textbf{KD-600} & \textbf{KD-900} & \textbf{RF+AEM} & \textbf{KD-300} & \textbf{KD-600} & \textbf{KD-900} & \textbf{RF+AEM} & \textbf{KD-300} & \textbf{KD-600} & \textbf{KD-900} \\
  
\midrule
\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}
&86.23&86.69&87.23&\textbf{87.56}
&70.68&71.62&72.21&\textbf{73.48}
&49.98&50.86&\textbf{52.49}&51.48\\
\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}
&78.97&77.98&80.53&\textbf{81.45}
&83.30&83.27&82.99&\textbf{84.14}
&78.33&78.94&79.07&\textbf{79.32}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}
&78.44&78.82&80.64&\textbf{81.35}
&66.57&64.98&67.03&\textbf{69.95}
&40.91&40.16&\textbf{42.83}&42.29\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\circ$}
&87.59&88.58&\textbf{88.81}&88.56
&69.98&71.15&\textbf{72.55}&71.91
&45.35&44.43&\textbf{45.68}&44.23\\
\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&88.56&88.91&\textbf{88.98}&88.95
&85.24&\textbf{85.75}&84.94&85.19
&80.24&80.75&77.97&\textbf{81.83}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}
&82.04&82.87&83.29&\textbf{83.71}
&83.33&84.10&84.01&\textbf{84.58}
&79.56&\textbf{83.11}&81.24&81.45\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}
&90.24&90.42&90.44&\textbf{90.49}
&\textbf{75.12}&72.79&74.57&74.14
&47.51&44.97&\textbf{50.12}&49.31\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}
&88.32&88.71&\textbf{89.00}&88.83
&72.97&72.04&\textbf{73.04}&\textbf{74.04}
&50.40&51.48&53.81&\textbf{53.92}\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}
&90.37&90.20&\textbf{90.46}&90.37
&74.37&75.32&75.53&\textbf{75.83}
&54.20&51.56&52.96&\textbf{54.26}\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}
&\textbf{90.44}&90.28&90.29&90.42
&85.52&86.19&85.90&\textbf{86.21}
&79.28&\textbf{81.20}&80.57&80.44\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}
&91.01&90.98&\textbf{91.09}&91.05
&85.08&85.85&85.74&\textbf{85.92}
&82.40&83.10&\textbf{84.50}&82.01\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}
&90.92&90.86&\textbf{91.05}&90.87
&75.32&74.74&75.34&\textbf{75.51}
&52.44&51.71&\textbf{52.79}&\textbf{52.79}\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&89.19&91.11&91.03&\textbf{91.15}
&85.39&85.83&86.04&\textbf{86.11}
&79.61&81.49&78.92&\textbf{82.41}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&89.19&89.30&\textbf{89.40}&89.33
&83.95&84.48&84.78&\textbf{84.92}
&81.65&\textbf{82.33}&80.66&82.30\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&\textbf{91.49}&91.09&91.18&91.29
&85.15&85.31&\textbf{86.18}&85.91
&82.73&\textbf{83.18}&81.64&82.09\\
\midrule
\multicolumn{4}{c|}{\textbf{Average}}
&87.67&87.79&88.19&\textbf{88.36}
&78.80&78.89&79.39&\textbf{79.86}
&65.64&65.95&66.35&\textbf{66.67}\\

\bottomrule
\end{tabular}
\end{adjustbox}

\label{table:KD_detail_RFNet}
\vspace{-2mm}
\end{table*}

==> Tables/ablation_KD_detail_Robust.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\large
\renewcommand\arraystretch{1} 
\caption{The ablation study to evaluate the impact of increasing the training iterations of the knowledge distillation (KD)-based post-training method. We denote the models post-trained with $N$ epochs using the KD approach as KD-$N$. We compared the performance of our proposed method to the ROBUSTSEG\cite{chen2019robust} baseline. Results are reported using the Dice Score (\%) metric with BRATS2020. The available and missing modalities are denoted by \textbf{$\bullet$} and \textbf{$\circ$}, respectively.}
\begin{adjustbox}{width=2\columnwidth,center}
\begin{tabular}{cccc|cccc|cccc|cccc}
\toprule
\multicolumn{4}{c|}{}                                                                                                                                  & \multicolumn{12}{c}{\textbf{Dice score(\%)}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{5-16} 
\multicolumn{4}{c|}{\multirow{-2}{*}{\textbf{Modality}}}                                                                                               & \multicolumn{4}{c|}{\textbf{Whole}}                                                                                                                                                                        & \multicolumn{4}{c|}{\textbf{Core}}                                                                                                                                                                         & \multicolumn{4}{c}{\textbf{Enhancing}}                                                                                                                                                                     \\
\midrule
  
\textbf{Flair} & \textbf{T1} & \textbf{T1ce} & \textbf{T2} & \textbf{RS+AEM} & \textbf{KD-300} & \textbf{KD-600} & \textbf{KD-900} & \textbf{RS+AEM} & \textbf{KD-300} & \textbf{KD-600} & \textbf{KD-900} & \textbf{RS+AEM} & \textbf{KD-300} & \textbf{KD-600} & \textbf{KD-900} \\
  
\midrule
\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}
&\textbf{82.99}&82.31&82.33&82.39
&62.12&62.29&\textbf{62.84}&62.75
&\textbf{39.19}&39.08&38.09&38.85\\
\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}
&66.68&69.04&69.70&\textbf{69.91}
&74.93&75.79&76.89&\textbf{77.96}
&66.09&66.89&67.83&\textbf{69.42}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}
&64.29&67.26&67.53&\textbf{68.06}
&50.20&50.00&52.01&\textbf{53.74}
&24.22&23.82&25.06&\textbf{26.43}\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\circ$}
&\textbf{82.16}&80.89&80.53&80.27
&\textbf{58.69}&56.76&57.13&56.87
&\textbf{33.05}&32.23&32.20&32.26\\
\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&85.73&85.43&86.05&\textbf{86.29}
&83.05&83.05&83.66&\textbf{84.27}
&73.81&74.48&74.27&\textbf{74.77}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}
&73.57&74.94&75.09&\textbf{75.25}
&79.85&79.65&80.21&\textbf{80.39}
&73.35&73.32&74.37&\textbf{74.41}\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}
&86.54&86.62&86.90&\textbf{87.07}
&66.11&66.33&67.05&\textbf{67.87}
&38.32&37.67&37.87&\textbf{38.79}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}
&85.44&86.10&\textbf{86.40}&86.11
&67.33&68.09&68.68&\textbf{68.69}
&40.98&42.10&41.99&\textbf{42.50}\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}
&\textbf{88.23}&87.52&87.58&87.53
&67.99&67.64&68.11&\textbf{68.31}
&\textbf{42.80}&42.16&42.17&42.33\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}
&86.64&86.62&87.26&\textbf{87.42}
&81.74&82.26&82.71&\textbf{83.30}
&69.64&69.13&70.33&\textbf{70.76}\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}
&87.81&87.73&88.08&\textbf{88.30}
&82.77&83.46&83.60&\textbf{84.10}
&\textbf{73.27}&72.28&72.47&72.80\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}
&88.91&88.92&89.30&\textbf{89.36}
&70.24&70.58&71.03&\textbf{71.60}
&43.38&43.57&43.65&\textbf{44.27}\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&88.98&89.26&\textbf{89.55}&\textbf{89.55}
&83.02&83.65&83.97&\textbf{84.43}
&71.51&71.71&72.88&\textbf{73.27}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&86.43&86.54&86.93&\textbf{87.07}
&83.66&84.33&84.48&\textbf{84.88}
&75.41&\textbf{75.66}&75.35&75.23\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&89.08&89.58&89.87&\textbf{89.93}
&83.50&84.46&84.68&\textbf{85.03}
&73.70&73.90&74.06&\textbf{74.44}\\

\midrule
\multicolumn{4}{c|}{\textbf{Average}}
&82.90&83.25&83.54&\textbf{83.63}
&73.01&73.22&73.80&\textbf{74.28}
&55.91&55.87&56.17&\textbf{56.70}\\

\bottomrule
\end{tabular}
\end{adjustbox}

\label{table:KD_detail_Robust}
\vspace{-2mm}
\end{table*}

==> Tables/ablation_KD_detail_UHVED.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\large
\renewcommand\arraystretch{1} 
\caption{The ablation study to evaluate the impact of increasing the training iterations of the knowledge distillation (KD)-based post-training method. We denote the models post-trained with $N$ epochs using the KD approach as KD-$N$. We compared the performance of our proposed method to the UHVED\cite{dorent2019hetero} baseline. Results are reported using the Dice Score (\%) metric with BRATS2020. The available and missing modalities are denoted by \textbf{$\bullet$} and \textbf{$\circ$}, respectively.}
\begin{adjustbox}{width=2\columnwidth,center}
\begin{tabular}{cccc|cccc|cccc|cccc}
\toprule
\multicolumn{4}{c|}{}                                                                                                                                  & \multicolumn{12}{c}{\textbf{Dice score(\%)}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{5-16} 
\multicolumn{4}{c|}{\multirow{-2}{*}{\textbf{Modality}}}                                                                                               & \multicolumn{4}{c|}{\textbf{Whole}}                                                                                                                                                                        & \multicolumn{4}{c|}{\textbf{Core}}                                                                                                                                                                         & \multicolumn{4}{c}{\textbf{Enhancing}}                                                                                                                                                                     \\
\midrule
  
\textbf{Flair} & \textbf{T1} & \textbf{T1ce} & \textbf{T2} & \textbf{UH+AEM} & \textbf{KD-300} & \textbf{KD-600} & \textbf{KD-900} & \textbf{UH+AEM} & \textbf{KD-300} & \textbf{KD-600} & \textbf{KD-900} & \textbf{UH+AEM} & \textbf{KD-300} & \textbf{KD-600} & \textbf{KD-900} \\
  
\midrule
\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}
&78.60&79.58&80.26&\textbf{80.85}
&62.45&62.89&63.07&\textbf{63.78}
&37.81&38.18&38.27&\textbf{38.88}\\
\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}
&64.90&66.19&66.24&\textbf{67.41}
&73.83&74.50&74.06&\textbf{75.15}
&63.00&63.93&64.20&\textbf{65.31}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}
&\textbf{62.00}&61.52&61.50&61.69
&49.19&49.60&\textbf{50.57}&50.50
&22.31&23.08&\textbf{24.39}&24.24\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\circ$}
&79.60&80.41&80.11&\textbf{80.74}
&55.17&56.55&57.69&\textbf{57.91}
&25.08&26.82&29.82&\textbf{30.98}\\
\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&82.20&82.23&83.03&\textbf{83.32}
&80.58&79.94&80.43&\textbf{80.68}
&68.40&67.90&68.38&\textbf{68.99}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}
&70.79&70.76&70.59&\textbf{70.93}
&\textbf{78.08}&77.11&77.66&77.82
&67.04&66.96&67.23&\textbf{67.74}\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}
&83.24&83.76&83.26&\textbf{83.80}
&62.44&63.37&63.67&\textbf{64.05}
&32.84&33.30&34.87&\textbf{34.94}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}
&81.72&80.95&81.62&\textbf{82.08}
&\textbf{65.40}&64.92&64.92&65.27
&39.23&\textbf{39.64}&38.32&38.69\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\circ$}&\textbf{$\bullet$}
&83.64&84.11&84.24&\textbf{84.99}
&65.19&65.12&65.49&\textbf{65.85}
&40.80&40.71&41.04&\textbf{41.21}\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\circ$}
&83.05&84.09&84.30&\textbf{84.86}
&77.58&77.59&78.00&\textbf{78.42}
&67.01&\textbf{67.32}&67.10&67.21\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}
&84.39&85.07&85.23&\textbf{65.69}
&79.02&79.08&79.34&\textbf{79.84}
&67.84&68.08&68.19&\textbf{68.34}\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}
&85.28&85.42&85.67&\textbf{86.24}
&68.29&67.77&68.16&\textbf{68.51}
&41.25&\textbf{41.58}&41.16&41.27\\
\textbf{$\bullet$}&\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&85.41&86.07&86.51&\textbf{86.91}
&79.79&79.62&79.67&\textbf{79.94}
&67.42&67.38&67.63&\textbf{67.78}\\
\textbf{$\circ$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&83.31&82.27&83.44&\textbf{83.61}
&\textbf{81.08}&80.09&80.45&80.58
&69.02&68.58&68.81&\textbf{69.19}\\
\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}&\textbf{$\bullet$}
&85.97&86.30&87.01&\textbf{87.33}
&80.56&80.17&80.47&\textbf{80.67}
&67.89&67.86&68.14&\textbf{68.23}\\
\midrule
\multicolumn{4}{c|}{\textbf{Average}}
&79.61&79.95&80.20&\textbf{80.70}
&70.58&70.56&70.91&\textbf{71.27}
&51.80&52.09&52.50&\textbf{52.87}\\

\bottomrule
\end{tabular}
\end{adjustbox}

\label{table:KD_detail_UHVED}
\vspace{-2mm}
\end{table*}

==> Tables/mixup_and_aem_simple.tex <==
\begin{table}[h]
\caption{Average performance on BRAST2020 between two data augmentation methods.}
\centering
\begin{tabular}{l|l|l|l} 
\hline
\textbf{Method}        & \textbf{Whole}        & \textbf{Core}         & \textbf{Enhancing}     \\ 
\hline
UHVED        & 79.06        & 66.67        & 48.41         \\
UHVED+MIXUP    & \textbf{80.83$_{\color{red}{+1.77}}$} & 69.00$_{\color{red}{+2.33}}$ & 50.00$_{\color{red}{+1.59}}$   \\
UHVED+AEM & 79.61$_{\color{red}{+0.55}}$ & \textbf{70.58$_{\color{red}{+3.91}}$} & \textbf{51.80$_{\color{red}{+3.39}}$}  \\ 
\hline
RobustSeg        & 82.29        & 71.36        & 55.22         \\
RobustSeg+MIXUP    & 82.81$_{\color{red}{+0.52}}$  & 72.72$_{\color{red}{+1.36}}$ & 55.69$_{\color{red}{+0.47}}$  \\
RobustSeg+AEM & \textbf{82.90$_{\color{red}{+0.61}}$}  & \textbf{73.01$_{\color{red}{+1.65}}$} & \textbf{55.91$_{\color{red}{+0.69}}$}   \\ 
\hline
RFNet         & 86.81         & 78.65        & 64.11         \\
RFNet+MIXUP     & 86.52$_{\color{blue}{-0.29}}$ & 78.46$_{\color{blue}{-0.19}}$  & 64.31$_{\color{red}{+0.20}}$  \\
RFNet+AEM  & \textbf{87.67$_{\color{red}{+0.86}}$} & \textbf{78.80$_{\color{red}{+0.15}}$}  & \textbf{65.64$_{\color{red}{+1.53}}$}  \\
\hline
\end{tabular}
\label{table:mixup_and_aem_simple}
\end{table}


==> Tables/settings.tex <==
% \usepackage{tabularray}
\begin{table}
\caption{Detailed settings during different stages.}
\centering
\begin{tblr}{
  cells = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=2}{},
  cell{1}{5} = {r=2}{},
  vline{2-4} = {1-2}{},
  vline{4-5} = {1-2}{},
  vline{2-3,5} = {3-7}{},
  hline{1,3,8} = {-}{},
  hline{2} = {3-4}{},
  hline{4-7} = {1}{},
}
Settings      & Baseline & Data augmentation &          & {Knowledge \\Distill } \\
              &          & pre-train         & finetune &                        \\
Optimizer     & Adam     & Adam              & Adam     & Adam                   \\
learning rate & 2e-4     & 2e-4              & 2e-4     & 2e-4                   \\
wight decay         & 1e-4      & 1e-4&1e-4&1e-4           \\
batch-size    & 1        & 1                 & 1        & 1                      \\
iterations      &135000&90000&45000&135000\\
\end{tblr}
\label{table:settings}
\end{table}

==> Tables/soa_2015_simple.tex <==
\begin{table}[t]
\centering\small
\caption{The average performance of the proposed and the state-of-the-art approaches on BRATS2015. All results are reported with Dice Score (\%).}
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\toprule
Methods & Whole & Core & Enhancing \\ \midrule
HeMIS & 68.22 & 54.07 & 43.86 \\
U-HVED & 81.57 & 64.68 & 56.76 \\
RobustSeg & 84.45 & 69.19 & 57.33 \\
RFNet & 86.13 & 71.93 & 64.13 \\ \midrule
\textbf{Ours} & \textbf{86.97} & \textbf{73.75} & \textbf{65.86} \\
\bottomrule
\end{tabular}
}

	\label{table:soa_2015_simple} 	
\end{table}

==> Tables/soa_2020.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[t]
% \centering
% \small
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{ccccccccccccccccccc}
% \rowcolor[HTML]{B4C7E7} 
% \multicolumn{4}{c}{\cellcolor[HTML]{B4C7E7}} & \multicolumn{15}{c}{\cellcolor[HTML]{B4C7E7}\textbf{Dice Score(\%)}} \\
% \rowcolor[HTML]{B4C7E7} 
% \multicolumn{4}{c}{\multirow{-2}{*}{\cellcolor[HTML]{B4C7E7}\textbf{Modalities}}} & \multicolumn{5}{c}{\cellcolor[HTML]{B4C7E7}\textbf{Whole}} & \multicolumn{5}{c}{\cellcolor[HTML]{B4C7E7}\textbf{Core}} & \multicolumn{5}{c}{\cellcolor[HTML]{B4C7E7}\textbf{Enhancing}} \\
% \rowcolor[HTML]{B4C7E7} 
% \textbf{Flair} & \textbf{T1} & \textbf{T1ce} & \textbf{T2} & \textbf{HeMIS} & \textbf{U-HVED} & \textbf{RobustSeg} & \textbf{RFNet} & \textbf{Ours} & \textbf{HeMIS} & \textbf{U-HVED} & \textbf{RobustSeg} & \textbf{RFNet} & \textbf{Ours} & \textbf{HeMIS} & \textbf{U-HVED} & \textbf{RobustSeg} & \textbf{RFNet} & \textbf{Ours} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\bullet$} & 79.85 & 77.34 & 83.46 & 86.02 & {\color[HTML]{D83931} \textbf{87.56}} & 54.22 & 63.16 & 59.83 & 70.63 & {\color[HTML]{D83931} \textbf{73.48}} & 31.43 & 30.37 & 36.06 & 47.44 & {\color[HTML]{D83931} \textbf{51.48}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\circ$} & 64.58 & 62.88 & 70.49 & 76.23 & {\color[HTML]{D83931} \textbf{81.45}} & 69.41 & 69.35 & 74.78 & 82.36 & {\color[HTML]{D83931} \textbf{84.14}} & 63.24 & 60.28 & 66.34 & 73.53 & {\color[HTML]{D83931} \textbf{79.32}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\circ$} & 63.01 & 59.18 & 65.78 & 76.05 & {\color[HTML]{D83931} \textbf{81.35}} & 42.42 & 42.73 & 46.13 & 63.49 & {\color[HTML]{D83931} \textbf{69.95}} & 16.53 & 12.33 & 21.83 & 36.95 & {\color[HTML]{D83931} \textbf{42.29}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\circ$} & 52.29 & 79.22 & 83.69 & 87.35 & {\color[HTML]{D83931} \textbf{88.56}} & 24.97 & 59.30 & 59.47 & 68.91 & {\color[HTML]{D83931} \textbf{71.91}} & 9.00 & 22.51 & 34.39 & 39.75 & {\color[HTML]{D83931} \textbf{44.23}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\bullet$} & 84.45 & 80.31 & 86.57 & 87.49 & {\color[HTML]{D83931} \textbf{88.95}} & 77.60 & 76.65 & 82.45 & 85.04 & {\color[HTML]{D83931} \textbf{85.19}} & 70.30 & 63.38 & 72.23 & 75.78 & {\color[HTML]{D83931} \textbf{81.83}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\circ$} & 72.50 & 66.69 & 74.65 & 80.41 & {\color[HTML]{D83931} \textbf{83.71}} & 75.59 & 73.97 & 78.03 & 82.86 & {\color[HTML]{D83931} \textbf{84.58}} & 70.71 & 63.17 & 68.86 & 76.72 & {\color[HTML]{D83931} \textbf{81.45}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\circ$} & 65.29 & 81.74 & 87.09 & 89.74 & {\color[HTML]{D83931} \textbf{90.49}} & 41.58 & 64.81 & 65.62 & 71.70 & {\color[HTML]{D83931} \textbf{74.14}} & 13.99 & 25.12 & 37.87 & 46.33 & {\color[HTML]{D83931} \textbf{49.31}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\bullet$} & 82.31 & 79.82 & 85.63 & 87.87 & {\color[HTML]{D83931} \textbf{88.83}} & 56.38 & 64.93 & 66.19 & 72.53 & {\color[HTML]{D83931} \textbf{74.04}} & 28.58 & 31.13 & 39.29 & 49.73 & {\color[HTML]{D83931} \textbf{53.92}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\bullet$} & 81.56 & 82.78 & 88.37 & 89.56 & {\color[HTML]{D83931} \textbf{90.37}} & 55.89 & 67.09 & 67.40 & 73.23 & {\color[HTML]{D83931} \textbf{75.83}} & 28.91 & 28.42 & 42.26 & 49.71 & {\color[HTML]{D83931} \textbf{54.26}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\circ$} & 69.37 & 82.42 & 87.79 & 89.56 & {\color[HTML]{D83931} \textbf{90.42}} & 70.86 & 76.64 & 81.20 & 85.42 & {\color[HTML]{D83931} \textbf{86.21}} & 68.31 & 63.93 & 70.09 & 75.70 & {\color[HTML]{D83931} \textbf{80.44}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\circ$} & 73.31 & 83.31 & 88.28 & 90.46 & {\color[HTML]{D83931} \textbf{91.05}} & 75.07 & 78.37 & 81.20 & {\color[HTML]{D83931} \textbf{86.04}} & 85.92 & 70.80 & 64.65 & 71.26 & 79.04 & {\color[HTML]{D83931} \textbf{82.01}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\bullet$} & 83.03 & 83.71 & 88.83 & 90.38 & {\color[HTML]{D83931} \textbf{90.87}} & 57.40 & 68.22 & 69.10 & 74.12 & {\color[HTML]{D83931} \textbf{75.51}} & 29.53 & 30.17 & 43.83 & 52.40 & {\color[HTML]{D83931} \textbf{52.79}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\bullet$} & \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\bullet$} & 84.64 & 84.14 & 89.49 & 90.41 & {\color[HTML]{D83931} \textbf{91.15}} & 77.69 & 78.30 & 82.52 & 85.43 & {\color[HTML]{D83931} \textbf{86.11}} & 71.36 & 64.77 & 71.86 & 78.14 & {\color[HTML]{D83931} \textbf{82.41}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\bullet$} & 85.19 & 81.09 & 86.46 & 88.21 & {\color[HTML]{D83931} \textbf{89.33}} & 79.05 & 78.42 & 83.02 & {\color[HTML]{D83931} \textbf{85.26}} & 84.92 & 71.67 & 64.53 & 71.86 & 79.24 & {\color[HTML]{D83931} \textbf{82.30}} \\
% \rowcolor[HTML]{DEEBF7} 
% \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\bullet$} & 85.19 & 84.56 & 89.54 & 90.90 & {\color[HTML]{D83931} \textbf{91.29}} & 78.58 & 79.43 & 82.65 & 85.90 & {\color[HTML]{D83931} \textbf{85.91}} & 71.49 & 65.29 & 71.37 & 79.26 & {\color[HTML]{D83931} \textbf{82.09}} \\
% \rowcolor[HTML]{DEEBF7} 
% \multicolumn{4}{c}{\cellcolor[HTML]{DEEBF7}\textbf{Average}} & 75.10 & 77.95 & 83.75 & 86.71 & {\color[HTML]{D83931} \textbf{88.36}} & 65.45 & 69.43 & 71.97 & 78.19 & {\color[HTML]{D83931} \textbf{79.86}} & 47.73 & 46.00 & 54.62 & 62.65 & {\color[HTML]{D83931} \textbf{66.67}}
% \end{tabular}
% }
% \caption{Comparisons with the state-of-the-art methods, including HeMIS\cite{}, U-HVED\cite{}, RobustSeg\cite{}, and RFNet\cite{} on BRATS2020. Whole, Core and Enhancing denote the Dice scores of the whole tumor, the tumor core and the enhancing tumor, respectively. All the results are reproduced by using the authors’ codes.}
% \end{table*}

\begin{table*}[]
\Huge
\renewcommand\arraystretch{1} 
\begin{adjustbox}{width=2\columnwidth,center}
\begin{tabular}{cccc|ccccc|ccccc|ccccc}
\toprule
\multicolumn{4}{c|}{}                                                                                                                                  & \multicolumn{15}{c}{\textbf{Dice score(\%)}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{5-19} 
\multicolumn{4}{c|}{\multirow{-2}{*}{\textbf{Modality}}}                                                                                               & \multicolumn{5}{c|}{\textbf{Whole}}                                                                                                                                                                        & \multicolumn{5}{c|}{\textbf{Core}}                                                                                                                                                                         & \multicolumn{5}{c}{\textbf{Enhancing}}                                                                                                                                                                     \\
\midrule

{\textbf{Flair}} & {\textbf{T1}} & {\textbf{T1ce}} & {\textbf{T2}} & {\textbf{HeMIS}} & {\textbf{U-HVED}} & {\textbf{RobustSeg}} & {\textbf{RFNet}} & {\textbf{Ours}} & {\textbf{HeMIS}} & {\textbf{U-HVED}} & {\textbf{RobustSeg}} & {\textbf{RFNet}} & {\textbf{Ours}} & {\textbf{HeMIS}} & {\textbf{U-HVED}} & {\textbf{RobustSeg}} & {\textbf{RFNet}} & {\textbf{Ours}} \\
\midrule
\textbf{$\circ$}                            & \textbf{$\circ$}                         & \textbf{$\circ$}                           & \textbf{$\bullet$}                         & 79.85                                 & 77.34                                  & 83.46                                      & 86.02                                 & \textbf{87.56}                       & 54.22                                 & 63.16                                  & 59.83                                      & 70.63                                 & \textbf{73.48}                       & 31.43                                 & 30.37                                  & 36.06                                      & 47.44                                 & \textbf{51.48}                       \\
\textbf{$\circ$}                            & \textbf{$\circ$}                         & \textbf{$\bullet$}                           & \textbf{$\circ$}                         & 64.58                                 & 62.88                                  & 70.49                                      & 76.23                                 & \textbf{81.45}                       & 69.41                                 & 69.35                                  & 74.78                                      & 82.36                                 & \textbf{84.14}                       & 63.24                                 & 60.28                                  & 66.34                                      & 73.53                                 & \textbf{79.32}                       \\
\textbf{$\circ$}                            & \textbf{$\bullet$}                         & \textbf{$\circ$}                           & \textbf{$\circ$}                         & 63.01                                 & 59.18                                  & 65.78                                      & 76.05                                 & \textbf{81.35}                       & 42.42                                 & 42.73                                  & 46.13                                      & 63.49                                 & \textbf{69.95}                       & 16.53                                 & 12.33                                  & 21.83                                      & 36.95                                 & \textbf{42.29}                       \\
\textbf{$\bullet$}                            & \textbf{$\circ$}                         & \textbf{$\circ$}                           & \textbf{$\circ$}                         & 52.29                                 & 79.22                                  & 83.69                                      & 87.35                                 & \textbf{88.56}                       & 24.97                                 & 59.30                                  & 59.47                                      & 68.91                                 & \textbf{71.91}                       & 9.00                                  & 22.51                                  & 34.39                                      & 39.75                                 & \textbf{44.23}                       \\
\textbf{$\circ$}                            & \textbf{$\circ$}                         & \textbf{$\bullet$}                           & \textbf{$\bullet$}                         & 84.45                                 & 80.31                                  & 86.57                                      & 87.49                                 & \textbf{88.95}                       & 77.60                                 & 76.65                                  & 82.45                                      & 85.04                                 & \textbf{85.19}                       & 70.30                                 & 63.38                                  & 72.23                                      & 75.78                                 & \textbf{81.83}                       \\
\textbf{$\circ$}                            & \textbf{$\bullet$}                         & \textbf{$\bullet$}                           & \textbf{$\circ$}                         & 72.50                                 & 66.69                                  & 74.65                                      & 80.41                                 & \textbf{83.71}                       & 75.59                                 & 73.97                                  & 78.03                                      & 82.86                                 & \textbf{84.58}                       & 70.71                                 & 63.17                                  & 68.86                                      & 76.72                                 & \textbf{81.45}                       \\
\textbf{$\bullet$}                            & \textbf{$\bullet$}                         & \textbf{$\circ$}                           & \textbf{$\circ$}                         & 65.29                                 & 81.74                                  & 87.09                                      & 89.74                                 & \textbf{90.49}                       & 41.58                                 & 64.81                                  & 65.62                                      & 71.70                                 & \textbf{74.14}                       & 13.99                                 & 25.12                                  & 37.87                                      & 46.33                                 & \textbf{49.31}                       \\
\textbf{$\circ$}                            & \textbf{$\bullet$}                         & \textbf{$\circ$}                           & \textbf{$\bullet$}                         & 82.31                                 & 79.82                                  & 85.63                                      & 87.87                                 & \textbf{88.83}                       & 56.38                                 & 64.93                                  & 66.19                                      & 72.53                                 & \textbf{74.04}                       & 28.58                                 & 31.13                                  & 39.29                                      & 49.73                                 & \textbf{53.92}                       \\
\textbf{$\bullet$}                            & \textbf{$\circ$}                         & \textbf{$\circ$}                           & \textbf{$\bullet$}                         & 81.56                                 & 82.78                                  & 88.37                                      & 89.56                                 & \textbf{90.37}                       & 55.89                                 & 67.09                                  & 67.40                                      & 73.23                                 & \textbf{75.83}                       & 28.91                                 & 28.42                                  & 42.26                                      & 49.71                                 & \textbf{54.26}                       \\
\textbf{$\bullet$}                            & \textbf{$\circ$}                         & \textbf{$\bullet$}                           & \textbf{$\circ$}                         & 69.37                                 & 82.42                                  & 87.79                                      & 89.56                                 & \textbf{90.42}                       & 70.86                                 & 76.64                                  & 81.20                                      & 85.42                                 & \textbf{86.21}                       & 68.31                                 & 63.93                                  & 70.09                                      & 75.70                                 & \textbf{80.44}                       \\
\textbf{$\bullet$}                            & \textbf{$\bullet$}                         & \textbf{$\bullet$}                           & \textbf{$\circ$}                         & 73.31                                 & 83.31                                  & 88.28                                      & 90.46                                 & \textbf{91.05}                       & 75.07                                 & 78.37                                  & 81.20                                      & \textbf{86.04}                        & 85.92                                & 70.80                                 & 64.65                                  & 71.26                                      & 79.04                                 & \textbf{82.01}                       \\
\textbf{$\bullet$}                            & \textbf{$\bullet$}                         & \textbf{$\circ$}                           & \textbf{$\bullet$}                         & 83.03                                 & 83.71                                  & 88.83                                      & 90.38                                 & \textbf{90.87}                       & 57.40                                 & 68.22                                  & 69.10                                      & 74.12                                 & \textbf{75.51}                       & 29.53                                 & 30.17                                  & 43.83                                      & 52.40                                 & \textbf{52.79}                       \\
\textbf{$\bullet$}                            & \textbf{$\circ$}                         & \textbf{$\bullet$}                           & \textbf{$\bullet$}                         & 84.64                                 & 84.14                                  & 89.49                                      & 90.41                                 & \textbf{91.15}                       & 77.69                                 & 78.30                                  & 82.52                                      & 85.43                                 & \textbf{86.11}                       & 71.36                                 & 64.77                                  & 71.86                                      & 78.14                                 & \textbf{82.41}                       \\
\textbf{$\circ$}                            & \textbf{$\bullet$}                         & \textbf{$\bullet$}                           & \textbf{$\bullet$}                         & 85.19                                 & 81.09                                  & 86.46                                      & 88.21                                 & \textbf{89.33}                       & 79.05                                 & 78.42                                  & 83.02                                      & \textbf{85.26}                        & 84.92                                & 71.67                                 & 64.53                                  & 71.86                                      & 79.24                                 & \textbf{82.30}                       \\
\textbf{$\bullet$}                            & \textbf{$\bullet$}                         & \textbf{$\bullet$}                           & \textbf{$\bullet$}                         & 85.19                                 & 84.56                                  & 89.54                                      & 90.90                                 & \textbf{91.29}                       & 78.58                                 & 79.43                                  & 82.65                                      & 85.90                                 & \textbf{85.91}                       & 71.49                                 & 65.29                                  & 71.37                                      & 79.26                                 & \textbf{82.09}                       \\
\midrule
\multicolumn{4}{c|}{\textbf{Average}}                                                                                                                   & 75.10                                 & 77.95                                  & 83.75                                      & 86.71                                 & \textbf{88.36}                       & 65.45                                 & 69.43                                  & 71.97                                      & 78.19                                 & \textbf{79.86}                       & 47.73                                 & 46.00                                  & 54.62                                      & 62.65                                 & \textbf{66.67}                                                   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Comparisons with the state-of-the-art methods, including HeMIS\cite{}, U-HVED\cite{}, RobustSeg\cite{}, and RFNet\cite{} on BRATS2020. Whole, Core and Enhancing denote the Dice scores of the whole tumor, the tumor core and the enhancing tumor, respectively. Results for HeMIS is taken from the original paper, and all other results are reproduced by using the authors’ codes.}
\label{table:soa_2020}
\end{table*}  
